JDOI Variance Reduction Method and the Pricing of American-Style Options

The present article revisits the Diffusion Operator Integral (DOI) variance reduction technique originally proposed in Heath and Platen (2002) and extends its theoretical concept to the pricing of American-style options under (time-homogeneous) L\'evy stochastic differential equations. The resulting Jump Diffusion Operator Integral (JDOI) method can be combined with numerous Monte Carlo based stopping-time algorithms, including the ubiquitous least-squares Monte Carlo (LSMC) algorithm of Longstaff and Schwartz (cf. Carriere (1996), Longstaff and Schwartz (2001)). We exemplify the usefulness of our theoretical derivations under a concrete, though very general jump-diffusion stochastic volatility dynamics and test the resulting LSMC based version of the JDOI method. The results provide evidence of a strong variance reduction when compared with a simple application of the LSMC algorithm and proves that applying our technique on top of Monte Carlo based pricing schemes provides a powerful way to speed-up these methods.

==> Arxiv Submission/acronyms.tex <==
%auto-ignore
\newacronym{doi}{DOI}{Diffusion Operator Integral}
\newacronym{lsmc}{LSMC}{Least-Squares Monte Carlo}
\newacronym{mc}{MC}{Monte Carlo}
\newacronym{gpr}{GPR}{Gaussian Process Regression}
\newacronym{sde}{SDE}{Stochastic Differential Equation}
\newacronym{fd}{FD}{Finite Difference}

==> Arxiv Submission/chapters/acronyms.tex <==
%auto-ignore
\newacronym{doi}{DOI}{Diffusion Operator Integral}
\newacronym{lsmc}{LSMC}{Least-Squares Monte Carlo}
\newacronym{mc}{MC}{Monte Carlo}
\newacronym{gpr}{GPR}{Gaussian Process Regression}
\newacronym{sde}{SDE}{Stochastic Differential Equation}

==> Arxiv Submission/chapters/packages.tex <==
%auto-ignore
% document properties
\usepackage[utf8]{inputenc}
\usepackage[left=.5in, right=.5in, top=1in, bottom=1in]{geometry}
\usepackage[american]{babel}
\usepackage{parskip}

% glossaries
\usepackage{glossaries}
\input{acronyms}

% tables
\usepackage{tabularx}
\usepackage{booktabs}

% lipsum for previews
\usepackage{lipsum}

% math
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{dsfont}

% number equations by section
\numberwithin{equation}{section}

% subfiles
\usepackage{subfiles}
% for cross-citations between subfiles
\usepackage{xr}


==> Arxiv Submission/packages.tex <==
%auto-ignore
% document properties
\usepackage[utf8]{inputenc}
\usepackage[left=.5in, right=.5in, top=1in, bottom=1in]{geometry}
\usepackage[american]{babel}
\usepackage{parskip}
\usepackage{float}
\usepackage[labelfont=bf]{caption}

% glossaries
\usepackage{glossaries}
\input{acronyms}

% tables
\usepackage{tabularx}
\usepackage{booktabs}

% lipsum for previews
\usepackage{lipsum}

% math
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{dsfont}
\usepackage{mathtools}

% number equations by section
\numberwithin{equation}{section}

% subfiles
\usepackage{subfiles}
% for cross-citations between subfiles
\usepackage{xr}

% bibliography
\usepackage[
backend=bibtex,
style=alphabetic,
citestyle=trad-alpha
]{biblatex}

%import bib-file
\addbibresource{mybib.bib}

% taken from the chapter about extension to Barriers,
% CHECK which packges are really needed
\usepackage{latexsym}
\usepackage{graphicx}
\usepackage{mathrsfs}
\usepackage{amsthm}
\usepackage{mdframed}
\usepackage{bbm}
\usepackage{color}
\usepackage{capt-of}
\usepackage{xcolor}

% command for comments
\newcommand\wip[1]{\textbf{\textcolor{red}{[#1]}}}

==> chapters/acronyms.tex <==
%auto-ignore
\newacronym{doi}{DOI}{Diffusion Operator Integral}
\newacronym{lsmc}{LSMC}{Least-Squares Monte Carlo}
\newacronym{mc}{MC}{Monte Carlo}
\newacronym{gpr}{GPR}{Gaussian Process Regression}
\newacronym{sde}{SDE}{Stochastic Differential Equation}

==> chapters/packages.tex <==
%auto-ignore
% document properties
\usepackage[utf8]{inputenc}
\usepackage[left=.5in, right=.5in, top=1in, bottom=1in]{geometry}
\usepackage[american]{babel}
\usepackage{parskip}

% glossaries
\usepackage{glossaries}
\input{acronyms}

% tables
\usepackage{tabularx}
\usepackage{booktabs}

% lipsum for previews
\usepackage{lipsum}

% math
\usepackage{amsfonts}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{dsfont}

% number equations by section
\numberwithin{equation}{section}

% subfiles
\usepackage{subfiles}
% for cross-citations between subfiles
\usepackage{xr}

